Normative Requirements Operationalization with Large Language Models

Normative non-functional requirements specify constraints that a system must observe in order to avoid violations of social, legal, ethical, empathetic, and cultural norms. As these requirements are typically defined by non-technical system stakeholders with different expertise and priorities (ethicists, lawyers, social scientists, etc.), ensuring their well-formedness and consistency is very challenging. Recent research has tackled this challenge using a domain-specific language to specify normative requirements as rules whose consistency can then be analysed with formal methods. In this paper, we propose a complementary approach that uses Large Language Models to extract semantic relationships between abstract representations of system capabilities. These relations, which are often assumed implicitly by non-technical stakeholders (e.g., based on common sense or domain knowledge), are then used to enrich the automated reasoning techniques for eliciting and analyzing the consistency of normative requirements. We show the effectiveness of our approach to normative requirements elicitation and operationalization through a range of real-world case studies.

==> Archive/background.tex <==
\section{Preliminaries}
\label{sec:background}

In this section, we present background material. In Sec.~\ref{ssec:ndsl}, we review the details of \dsl, and in Sec.~\ref{ssec:wfi}, we present well-formedness issues of SLEEC requirements.


%------------  Synthax
\begin{table}[t]
    \centering
    \caption{\small Syntax of normalized $\dsl$ with signature ($\events$, $\measures$).}
    \vspace{-0.1in}
    \scalebox{0.8}{
        \begin{tabular}{ll}
        \toprule
        Name & Definition\\
        \hline
        Term & $\term$ := $\constant :\mathbb{N} \mid \measure\in \measures \mid -\term \mid \term + \term \mid \constant \times \term$  \\
        Proposition & $\prop$ := $\top \mid \bot \mid \term = \term \mid \term \ge \term \mid \notS \; \prop \mid \prop \; \andS \; \prop \mid \prop \; \orS \; \prop$ \\
        Obligation & $\obg^+$ := $ \within{\event}{\term}$ $ \mid$ $\obg^-$ := $\within{\notS \; \event}{\term}$ \\
        Cond Obligation & $\cobg^+$ := $\prop \Rightarrow \obg^+$ $\mid$ $\cobg^-$ := $\prop \Rightarrow \obg^-$ \\
        Obligation Chain & $\dobg $ := $\cobg \mid \cobg^+ \otherwise \dobg$ \\
        Rule & $\srule $ := $\rulesyntax{\event \sand \prop }{\dobg}$ \\
        \hline
        Fact & $\fact$ := $\factsyntax{\event \sand \prop}{(\dobg \mid \notS \dobg)}$\\
        \bottomrule
        \\
        \end{tabular}
    }
 \label{tab:syntax}
 \vspace{-0.18in}
\end{table}

% header
%In this section, we overview the SoTA \dsl for specification of normative requirements and the \fol satisfiability checker. 

\subsection{Normalized Representation of \dsl}\label{ssec:ndsl}
% \hl{TODO:sleec dsl background}~\cite{Getir-Yaman-et-al-23}
 %The 
 \dsl is an event-based language for specifying normative requirements through the pattern ``\textbf{when} trigger \textbf{then} response'' ~\cite{Getir-Yaman-et-al-23}. It builds on propositional logic enriched with temporal constraints (e.g., \textbf{within} x \textbf{minutes}) and the constructs \textbf{unless}, specifying \emph{defeaters}, and \textbf{otherwise}, specifying \emph{fallbacks}.
 %, allowing complex nested logical structures for specifying responses.
%
% In the \dsl, 
% \emph{triggers} are based on the  occurrence of events and \blue{condition of values of measures (combined with propositional logics)}. {\bf MC:  not sure what prev sentence is saying} \green{\textbf{\underline{Better?}}} {\bf MC:  NOPE}
% \emph{Responses} restrict occurrences of events, specifying defeaters, deadlines, and fallback responses in case of timeouts.
% This allows responses to be specified via complex nested logical structures.
%\red{\textbf{NF: I commented out some sentences because I don't see why they need to be there}}
\dsl is an expressive language, allowing specification of complex nested defeaters and responses.
%\red{Due to \dsl's expressiveness for specifying complex nested defeaters}, 
A \dsl rule may be represented by multiple logically equivalent formulations, complicating analysis and reasoning.  This issue can be addressed with the \textit{normalized} \dsl here, which simplifies nested response frameworks and removes defeaters, encoding their semantics using propositional logic.
% 
A translation from \dsl to the normalized form is provided in~\cite{feng-et-al-24-e}.

\vspace{-0.05in}
\noindent
\boldparagraph{Normalized \dsl syntax}
A normalised \dsl \emph{signature} is a tuple $\sig = (\events, \measures)$, where $\events = \{\event_1, \ldots, \event_n\}$ and $\measures = \{\measure_1 \ldots \measure_n\}$ are finite sets of symbols  for \textit{events}  and \textit{measures}, respectively. In the rest of the paper, we assume that all event symbols (e.g., {\small \texttt{OpenCurtain}}) are capitalized while measure symbols (e.g., {\small \texttt{underDressed}}) are not. 
% , events start with a capital letter and measures -- with a lower case letter.
Without loss of generality, we assume that every measure is numerical. The syntax of the normalized \dsl{} can be found in Tbl.~\ref{tab:syntax}.  For example, an \textit{obligation} $\obg = \within{\obghead}{\term}$ specifies that the event $\event$ must (if $\obghead = \event$) or must not  (if $\obghead = \notS \; \event$) occur within the time limit $\term$. We omit the time limit $t$ if $t = 0$.
\begin{table}[t]
    \centering
    \caption{{\small Capabilities, definitions and requirements of  DAISY~\cite{daisy-22}.}}
    \label{tab:mainTable}
    \vspace{-0.02in}
    % Left side - two tables, one on top of the other
    \begin{minipage}{\linewidth}
        \centering
        % SLEEC definitions
        \begin{subtable}{\linewidth}
            \centering  
            \caption{{\small DAISY capabilities.}}
            \label{tab:capabilities}
            \scalebox{0.72}{
                \begin{tabular}{l l l}
                %\toprule
                %\multicolumn{3}{c}{a. DAISY Capabilities} \\
                \toprule
                - Meet a patient & - Issue commands to the patient & - Explain the protocols to the patient \\
                - Examine the patient & - Collect patient data & - Perform triage assessment \\
                - Provide instructions & - Repeat the instructions  & - Request clinician intervention \\
                \bottomrule
                \\
                \end{tabular}
            }
        \end{subtable}
        
        \vspace{0.1em} % Add some vertical space between the two tables
        
        % SLEEC definitions
        \begin{subtable}{\linewidth}
            \centering
            \caption{{\small Sample DAISY \dsl definitions.}}
            \label{tab:defs}
            \scalebox{0.9}{
                \begin{tabular}{cl | cl}
                %\toprule
                %\multicolumn{4}{c}{\dsl Definitions} \\
                \toprule
                \sleeckeyword{event} & 
                \sleec{ExamineState} & \sleeckeyword{measure} & \sleec{patientStressed} \\
                \sleeckeyword{event} & \sleec{IdentifyDAISYTrust} & \sleeckeyword{measure} & \sleec{patientAgeConsidered}  \\
                \sleeckeyword{event} & \sleec{MeetingUser}  & \sleeckeyword{measure} & \sleec{patientXReligion} \\
                \sleeckeyword{event} & \sleec{MeetingPatient}  & \sleeckeyword{measure} & \sleec{userDirectsOtherwise} \\
                \bottomrule
                \\
                \end{tabular}
            }   
            \vspace{0.1em} % Add some vertical space between the two tables

            % Requirements
    \begin{subtable}{\linewidth}
        \centering
        \caption{{\small Sample DAISY \dsl requirements.}}
        \label{tab:reqs}
        \scalebox{0.9}{
            \begin{tabular}{cl}
            %\toprule
            %\multicolumn{2}{c}{\dsl Requirements} \\
            \toprule
        	\sleec{Rule10} & \sleec{\sleeckeyword{when} MeetingUser \sleeckeyword{then} ExamineState} \\
        	\sleec{Rule13} & \sleec{\sleeckeyword{when} MeetingUser \sleeckeyword{then} IdentifyDAISYTrust} \\
            \sleec{Rule16} & \sleec{\sleeckeyword{when} MeetingUser \sleeckeyword{then} ExaminingPatient} \\
            & \sleec{\sleeckeyword{within} 30 \sleeckeyword{minutes} \sleeckeyword{unless} patientStressed} \\ 
            \sleec{Rule19} & \sleec{\sleeckeyword{when} MeetingUser \sleeckeyword{and} patientXReligion}\\
            & \sleec{\sleeckeyword{then not} ExaminingPatient} 
        	   \\
        	& \sleec{\sleeckeyword{unless} userDirectsOtherwise} \sleec{\sleeckeyword{unless} medicalEmergency} \\ 
            \bottomrule
            \\
            \end{tabular}
        }
    \end{subtable}
            
        \end{subtable}
    \end{minipage}
    \vspace{-0.4in}
\end{table}
\vspace{-0.05in}
\begin{example}\label{example:syntax}
Consider DAISY~\cite{daisy-22}, a sociotechnical AI-supported system to direct patients through an A\&E triage pathway. 
%Here
%we focus on the normative requirements related to the first interactions between DAISY and its users (patients). 
Tbl.~\ref{tab:capabilities} describes DAISY capabilities. 
One normative rule (\sleecT{Rule16}) is ``\sleecT{\sleeckeyword{when} MeetingUser \sleeckeyword{then} ExaminingPatient
\sleeckeyword{within} 30 \sleeckeyword{minutes} \sleeckeyword{unless} \sleeckeyword{patientStressed}}'', where \sleecT{MeetingUser} and \sleecT{ExaminingPatient} are events and \sleecT{patientStressed} a measure. \sleecT{Rule16} is normalized as ``\sleeckeyword{when} \sleecT{MeetingUser} \sleeckeyword{and not} \sleecT{patientStressed} \sleeckeyword{then} \sleecT{ExaminingPatient} \sleeckeyword{within} 30 \sleeckeyword{minutes}''.
\end{example}

\vspace{-0.1in}
\noindent
\boldparagraph{Semantics}
The semantics of \dsl is described over  \textit{traces}, which are \textit{finite} sequences of \textit{states} $\fos = (\eventocc{1}, \measureassign{1}, \timestamp{1}), (\eventocc{2}, \measureassign{2}, \timestamp{2}),$ $\ldots  (\eventocc{n}, \measureassign{n}, \timestamp{n})$. For every time point $i \in [1, n]$, (1) $\eventocc{i}$ is a set of events that occur at $i$; (2) $\measureassign{i}: \measures \rightarrow \mathbb{N}$ assigns every measure in $\measures$ to a concrete value at time point $i$, and (3) $\timestamp{i}: \mathbb{N}$ captures the value of time point $i$ (e.g., the second time point can have the value 30, for 30 sec). We assume that the time values in the trace are strictly increasing (i.e., $\timestamp{i} < \timestamp{i+1}$ for every $i \in [1, n-1]$). Given a measure assignment $\measureassign{i}$ and a term $\term$, let $\measureassign{i}(\term)$ denote the result of substituting every measure symbol $\measure$ with $\measureassign{i}(\measure)$. Since $\measureassign{i}(\term)$ does not contain free variables, the substitution results in a natural number. 
 Similarly, given a proposition $\prop$, we say that $\measureassign{i} \models \prop$ if $\prop$ is evaluated to $\top$ after substituting every term $\term$ with $\measureassign{i}(\term)$.  
%The complete semantics of \dsl can be found in Appendix.~\ref{sec:norm}. 
Let a trace $\fos = (\eventocc{1}, \measureassign{1}, \timestamp{1}) \ldots (\eventocc{n}, \measureassign{n}, \timestamp{n})$ be given.

\italicparagraph{Positive obligation} A positive obligation $\within{\event}{\term}$ is \textit{fulfilled subject to time point $i$}, denoted $\fos \models_{i} \within{\event}{\term}$, if there is a time point $j \ge i$ such that $e \in \eventocc{j}$ and $\timestamp{j} \in [\timestamp{i}, \timestamp{i} + \measureassign{i}(\term)]$. That obligation is \emph{violated at time point $j$}, denoted as $\fos \not\models_{i}^{j} \within{\event}{\term}$, if $\timestamp{j} = \timestamp{i} + \measureassign{i}(\term)$, and for every $j'$ such that $j \ge j' \ge i$, $\event$ does not occur ($\event \not\in \eventocc{j'}$).  

\italicparagraph{Negative obligation} A negative obligation $\within{\notS \; \event}{\term}$ is fulfilled subject to time point $i$, denoted as  $\fos \models_{i} \within{\notS \; \event}{\term}$, if for every time point $j$ such that $\timestamp{j} \in [\timestamp{i}, \timestamp{i} + \measureassign{i}(\term)]$, $e \not\in \eventocc{j}$. 
The negative obligation is violated at time point $j$, denoted as $\fos \not\models_{i}^{j} \within{\notS \; \event}{\term}$, if (1) $\timestamp{j} \in [\timestamp{i}, \;\timestamp{i} + \measureassign{i}(\term)]$, (2) $\event$ occurs ($\event \in \eventocc{j}$), and (3) for every $j \ge j' \ge i$, $\event$ does not occur ($\event \not\in \eventocc{j'}$). 

\italicparagraph{Conditional obligation} A conditional obligation $\prop \Rightarrow \obg$ is fulfilled subject to time point $i$, denoted as $\fos \models_{i} (\prop \Rightarrow \obg)$, if $\prop$ does not hold at time point $i$ (that is, $\measureassign{i}(\prop) = \bot$) or the obligation is fulfilled ($\fos \models_{i} \obg$).  Moreover, $\prop \Rightarrow \obg$  is violated at time point $j$, denoted as $\fos \not\models_{i}^{j} (\prop \Rightarrow \obg)$, if  $\prop$ holds at $i$ ($\measureassign{i}(\prop) = \top$) and $\obg$ is violated at $j$ ($\fos \not\models_{i}^{j} \obg$).

\vspace{-0.02in}
\italicparagraph{Obligation chain} A chain $\cobg^+_1 \otherwise \cobg^+_2 \ldots \cobg_m$ is fulfilled subject to time point $i$, denoted as $\fos \models_{i} \cobg^+_1 \otherwise$ $\cobg^+_2 \ldots \cobg_m$, if (1) the first obligation is fulfilled ($\fos \models_{i} \cobg^+_1$) or (2) 
there exists a time point $j \ge i$ such that $\cobg^+_1$ is \textit{violated} (i.e., $\fos \not\models_{i}^{j} \cobg_1$) and the rest of the obligation chain (if not empty) is fulfilled at time point $j$ ($\fos \models_{j} \cobg^+_2 \otherwise \ldots \cobg_m$).

\vspace{-0.02in}
\italicparagraph{Rule} A rule $\rulesyntax{\event \; \andS \; \prop}{\dobg}$ is fulfilled in $\fos$, denoted as $\fos \models \rulesyntax{\event \; \andS \; \prop}{\dobg}$, if for every time point $i$, 
where event $\event$ occurs ($\event \in \eventocc{i}$) and $\prop$ holds ($\measureassign{i}(\prop) = \top$), the obligation chain is fulfilled subject to time point $i$ ($\fos \models_{i} \dobg$). A \emph{trace fulfills a rule set} $\ruleset$, denoted as $\fos \models \ruleset$, if it fulfills every rule in the set (i.e., for every $\srule \in \ruleset$,  $\fos \models \srule$). 

% Figure
\input{Sections/figTraces}

\vspace{-0.05in}
\begin{example}
    Consider the normalized \dsl rule \sleecT{Rule16} in Example~\ref{example:syntax} and the trace $\sigma_1$ shown in Fig.~\ref{fig:trace}, corresponding to $(\eventocc{1}, \measureassign{1}, \timestamp{1})$, where $\eventocc{1} =$ \sleecT{MeetingUser}, $\measureassign{1}$(\sleecT{patientStressed}) = $\top$, and $\timestamp{1} = 1$. The trace $\sigma_1$ fulfills the rule \sleecT{Rule16}  (i.e., $\sigma_1 \models$ \sleecT{patientStressed}), because the rule's triggering condition  \sleecT{\sleeckeyword{not} patientStressed} is not satisfied, i.e., the patient is \sleecT{patientStressed} at the time of the meeting). 
\end{example}

\vspace{-0.11in}
\begin{definition}[Behaviour defined by $\ruleset$]\label{def:behav}
    Let a rule set  $\ruleset$ be given. The accepted \emph{behaviour} defined by $\ruleset$, denoted as $\lang{\ruleset}$, is the largest set of traces such that every trace $\fos$ in $\lang{\ruleset}$ respects  $\ruleset$, i.e., $\fos \in \lang{\ruleset}$, $\fos \models \ruleset$.
\end{definition}
    On top of the usual rules, \dsl also uses \emph{\facts} as an utility construct  describing the test scenarios for rules. A \emph{fact} (see Tab.~\ref{tab:syntax}) $\factsyntax{\event \wedge \prop}{(\dobg \mid \notS \dobg)}$ asserts the existence of an event $\event$ under condition $\prop$ while an obligation chain $\dobg$ is either satisfied  or violated. \facts~ can be used to describe undesirable behaviors, denoted as \textit{concerns}, which should be blocked by \dsl rules. Alternatively, \facts\; can also be used to describe functional goals, denoted as \textit{purposes}, which should be allowed by \dsl rules. 

\vspace{-0.05in{}}
\subsection{Well-Formedness Issues (\WFI)}
\label{ssec:wfi}
\dsl $\ruleset$ might be subject to well-formedness issues (WFIs): \emph{vacuous conflict},  \emph{redundancy}, \emph{insufficiency}, \emph{over-restrictiveness} and \emph{conditional conflict}. We  explain each WFI briefly and refer to~\cite{feng-et-al-24} for a formal definition.

\boldparagraph{Vacuous conflict} A rule is  \emph{vacuously conflicting in a rule set $\ruleset$} if triggering this rule always leads to a conflict with some other rules in $\ruleset$. 

\boldparagraph{Situational conflict} A rule is \emph{situational conflicting in a rule set $\ruleset$} if triggering this rule under a certain situation which defines a history of events and measures, always leads to a conflict with some other rules in the future.

\boldparagraph{Redundancy} A rule is  \emph{redundant in a rule set $\ruleset$} if this rule is logically implied by other rules in $\ruleset$.

\boldparagraph{Insufficiency} A rule set $\ruleset$ is \emph{insufficient subject to a given concern} if some behavior represented by the concern is realizable while respecting $\ruleset$.


\boldparagraph{Over-restrictiveness} A rule set $\ruleset$ is \emph{overly restrictive subject to a given purpose} if none of the functional goals represented by the purpose is realizable while respecting $\ruleset$.

 WFIs impose threats to the validity of \dsl rules. Conflicting rules must be resolved to avoid inevitable SLEEC harms. Insufficient  and  overly-restrictive rule sets also need to be fixed, to avoid executions of undesirable behaviors and violations of functional goals, respectively. Situational conflicts and redundancies also require attention. The former capture dead-end situations where conflicts become inevitable and the latter complicates  management of  evolving requirements.

\boldparagraph{Order of Resolving WFIs}
Different types of WFIs have different levels of severity and might depend on each other. 


Vacuous conflicts should be resolved prior to situational conflicts because any situation that triggers a vacuously conflicting rule will also create a conflicting situation. For example, consider \sleecT{R1 = \sleeckeyword{when} A \sleeckeyword{then} B}. This rule is vacuously conflicting due to another rule: \sleecT{R2 = \sleeckeyword{when} A \sleeckeyword{then} \sleeckeyword{not} B \sleeckeyword{within} 10 minutes}. This implies that $R1$ is also situationally conflicting since any situation that triggers $R1$ leads to a conflict. 
Insufficiency and over-restrictiveness are checked and resolved after both types of conflict because the behaviors defined by conflicting rules are inconsistent, and thus might affect the judgment of insufficiency or over-restrictiveness analysis. For example, without first resolving the vacuous or situational conflict between \sleecT{R1} and \sleecT{R2}, the conflicting situations are excluded from the insufficiency and over-restrictiveness analysis. The concern \sleecT{\sleeckeyword{exists} A \sleeckeyword{while} X} can never be identified in any currently conflicting situation (and cannot be identified at all if a vacuous conflict exists), thus it is blocked by the conflict.

 Redundancies are checked last because they are the least severe WFIs, and because they are affected by conflicts.  For example, without resolving the vacuous conflict between \sleecT{R1} and \sleecT{R2}, the rule \sleec{R3 = \sleeckeyword{when} A \sleeckeyword{then} C} is redundant because triggering \sleec{R3} would also trigger \sleec{R1} and subsequently cause a conflict. Moreover, the conflict subsumes the response of \sleec{R3} (e.g., \sleecT{C}), thus making the rule redundant.
 
% To summarize, the order in which WFIs should be checked and resolved is 
 %resolved in the following order:
%This is because fixing the cause or the blocker of WFIs might fix or reveal other WFIs, respectively. The dependencies suggest an order in which WFIs should be resolved:
%(1) vacuous conflicts, (2) situational conflicts, (3) insufficiencies and cases of over-restrictiveness, and (4) redundancies.
%    \item residencies.
%\end{enumerate}
%}
% \subsection{\tool}
\boldparagraph{\tool}~\cite{feng-et-al-24} was proposed to identify and resolve WFIs. It encodes the semantics of rules into \fol and turns WFI conditions into \fol satisfiability queries. The satisfiability results, either satisfying solutions or proofs of unsatisfiability, are then used to diagnose the causes of WFIs. 
\begin{example}
    Consider a rule set \sleec{Rules} $= \{$\sleec{Rule10}, \sleec{Rule10\_01}, \sleec{Rule10\_02}$\}$, where \sleec{Rule10,Rule10\_01,Rule10\_02} are rules in Tbl.~\ref{tab:reqs}.
    To check whether \sleec{Rule10} is redundant in \sleec{Rules}, we can use \tool which checks the satisfiability of the query $\{\neg$\sleec{Rule10} $\} \cup \{r \mid r \in$ \sleec{Rule10}$\setminus \{$\sleec{Rule10}$\}\}$. The query is unsatisfiable (UNSAT), which means that \sleec{Rule10} is a logical consequence of the $\{\neg$\sleec{Rule10}$\} \cup \{r \mid r \in$ \sleec{Rule10}; hence, \sleec{Rule10} is redundant. \tool provides a diagnosis shown in Fig.~\ref{fig:redundantDiag}, with the reason of redundancy highlighted.
\end{example}

\begin{figure}
    \centering \shadowbox{\includegraphics[width=0.47\textwidth,trim={0cm 0cm 0.8cm 0.1cm}, clip]{Sections/Img/RedundantDaisyDiag.png}}
    \caption{{\small Redundancy diagnosis example.}}
    \label{fig:redundantDiag}
    \vspace{-0.2in}
\end{figure}

==> Archive/introSUb.tex <==

\vspace{-0.05in}
\section{Introduction}


\hl{Define “common sense”, put it into context as it appears to be an important aspect of the defined problem.}

\hl{TODO: redo motivation - it is not about being able to formalize the common sense relationship but about to capture them in the first place, because the stakeholders do not realize that these relationship must be captured (implicit assumption), ILLUSTRATE THIS}

\hl{Improve the introduction to make clear what is the problem we are addressing to avoid this misunderstanding: The research goals must be explicitly formulated. Based on the introduction, my understanding is that this is a curiosity-driven study, i.e. the authors are interested in assessing the performance of disruptive technologies that is currently achieving state-of-the-art performance in several NLP tasks.}

% \hl{[Coming soon]}
% \hl{[Add intuition behind the name RAINCOAT]}
% Big context
Software systems are increasingly capable to perform daily tasks alongside humans, as important components of our infrastructure. Therefore, ensuring the \emph{responsible} integration of these systems into our society is becoming crucial. This includes preventing them from violating social, legal, ethical, empathetic, and cultural~(SLEEC) norms~\cite{townsend-et-al-2022,Getir-Yaman-et-al-23,Getir-Yaman-et-al-23b}. As such, it is important to elicit \emph{normative non-functional requirements}~(N-NFRs). %, which specify the permissible range of a system's behaviours. 
Due to the nature of the N-NFRs, their elicitation involves non-technical stakeholders (e.g., ethicists, lawyers), each with different and potentially conflicting jargon, goals, priorities, and responsibilities. So, it is particularly important to support the professionals in ensuring that the elicited N-NFRs do not have well-formedness issues (WFIs)~\cite{Getir-Yaman-et-al-23,feng-et-al-23-b,feng-et-al-24,Getir-Yaman-et-al-23b} such as conflict and redundancy~\cite{Getir-Yaman-et-al-23b}.
%, making the elicitation of a cohesive and well-formed set of requirements notoriously challenging

% Previous work
%To address this problem, 
Previous work has proposed a rule-based SLEEC language to formalize N-NFRs~\cite{Getir-Yaman-et-al-23}. Automated techniques, based on first-order logic~\cite{feng-et-al-23} and a process algebra~\cite{Gibson-Robinson-et-al-14,DBLP:journals/acta/BaxterRC22}, have been developed to check normative requirements specified in this language for WFIs~\cite{Getir-Yaman-et-al-23,Getir-Yaman-et-al-23b,feng-et-al-23-b,feng-et-al-24}. While effective, these techniques assume that all capabilities %resolved:\textbf{SGY: is the term capabilities common? i guess you refer the capabilities in SLEEC language?} 
referenced in the rules are independent. More precisely, the non-terminal symbols used for describing events and measures in the rules are treated as uninterpreted constants that do not carry semantics. However, in practice, many of these capabilities are related, if we take into account common sense or domain knowledge, and those relations are often assumed by non-technical stakeholders. For example, `on' and `off' measures of a camera can be reasonably expected to be mutually exclusive. Ignoring these semantic relations can affect the soundness and completeness of the WFI analysis. For example, consider the SLEEC rules:

\smallskip
\noindent
\hspace*{5mm} $r_1$ = \sleec{\sleeckeyword{when} BatteryLow \sleeckeyword{then} MuteNotifications}\\
\hspace*{5mm}
$r_2$ = \sleec{\sleeckeyword{when} BatteryLow \sleeckeyword{then} SendUserWarning }

\smallskip
\noindent
In the rule set $\{r_1, r_2\}$, $r_1$ is conflicting with $r_2$. This is because $r_1$ and $r_2$ share the same triggering event \sleec{BatteryLow}, and the response of $r_1$, \sleec{MuteNotifications}, is contradictory with the response of $r_2$, \sleec{SendUserWarning}. The contradiction follows from the fact that, if the events \sleec{MuteNotifications} and  \sleec{SendUserWarning} occur simultaneously, that is, in the same time unit, they cannot both have their intended effect. When all goes well (that is, there is no failure), either a warning is delivered, or the agent is muted, but not both. However, existing automated reasoning techniques~\cite{Getir-Yaman-et-al-23,feng-et-al-23-b,feng-et-al-24} 
fail to detect this conflict as they do not capture the semantic relation between the two events used in the responses. Therefore, there is a need to define and capture semantic relations of terms used in N-NFRs according to common sense and domain knowledge, and to use these relations in the N-NFR analysis.

Traditional knowledge extraction approaches may be considered as a means for addressing this need. However, they use as input (structured or unstructured) sources without information specific to applications, while the semantic relations for capabilities used in SLEEC requirements come from common sense in the context of domain-specific environments.
%
%, not does not come from the available sources (i.e., SLEEC requirements). Instead, they come from common sense and assumed domain-specific environments. 
Therefore, these knowledge extraction approaches are ineffective without an additional knowledge source, such as a domain-specific ontology~\cite{Farfeleder2005MKSO,Murugesh2015J,BencharquiOntologybasedRS, Diamantopoulos2018EnhancingRR} that is effort-intensive and costly to assemble. %\textbf{SGY: There is work on domain spesific knowledge graphs. maybe we dont need to mention this.} 
Our work addresses this issue without requiring such effort to structure the domain knowledge. To that end, we exploit the knowledge captured in Large Language Models (LLMs). LLMs are pre-trained with a vast amount of data covering a wide range of topics. They have been shown effective in answering questions regarding common sense~\cite{DBLP:conf/naacl/TalmorHLB19,DBLP:conf/aaai/BiskZLGC20,DBLP:journals/corr/abs-2303-11436} and domain-specific knowledge such as programming~\cite{DBLP:conf/aaai/JoshiSG0VR23,DBLP:conf/icer/PhungPCGKMSS22}, healthcare~\cite{DBLP:journals/jms/CascellaMBB23,haupt2023ai}, and law~\cite{DBLP:journals/corr/abs-2209-13020,DBLP:journals/corr/abs-2212-02199}. LLMs are also capable of obtaining new knowledge from analogies and examples~\cite{DBLP:conf/sigsoft/GuptaKBCGKRS023,DBLP:journals/corr/abs-2308-16118}. Therefore, we propose to use LLMs for suggesting potential semantic relations among system capabilities subject to SLEEC requirements. For the example above, GPT-4.0 successfully suggested that \sleec{MuteNotifications} is contradictory with \sleec{SendUserWarning}.

On the other hand, using LLMs comes with its own risks, as they are notorious for producing significantly incorrect results~\cite{DBLP:journals/corr/abs-2309-05922,DBLP:journals/corr/abs-2309-01219}. To prevent any falsely identified semantic relations from confounding WFI analysis, we also propose a lightweight logic-based filtering algorithm that incrementally extends relations via a set of inference rules and heuristically fixes logical inconsistencies on-the-fly. The filtered relations do not induce any logical fallacies and can be used directly for WFI analysis. We still, however, ask stakeholders to further filter the relations based on their domain-specific knowledge.

% Approach schema
\input{Sections/fig-approach}

%In addition to discovering and integrating semantic relations in SLEEC, 
%We propose here a tool-supported approach, \approach, for N-NFR requirement elicitation,
%using SLEEC and the additional reasoning component presented in this paper. 
%As depicted in Fig.~\ref{fig:approach}, 
%\approach is an iterative process with six stages defining the order of the analyses and their resolution strategies upon identification of WFIs. %resolved: \textbf{SGY: to what is it an alternative and why?} %For example, \approach prioritizes analyzing and resolving conflicts prior to redundancy since the former can trivially lead to later (i.e., `false' can logically imply everything).

% \hl{TODO: add a mini related work}.
To summarise, the main contributions of our paper are:
(1)
%\begin{enumerate}
%    \item 
    An LLM-based technique that extracts semantic relations between the capabilities of a system under development, where these capabilities appear as non-terminal symbols in the SLEEC rules that encode the system's N-NFRs; 
    (2) The integration of our new semantic-relation extraction technique 
with existing automated reasoning methods, to develop a systematic end-to-end approach, \approach, for eliciting and analyzing normative requirements; 
(3)  An extensive evaluation (with five non-technical stakeholders, using a range of real-world case studies) that shows the effectiveness and usability of our LLM-based technique and the \approach approach.

% Structure of the paper
The rest of the paper is organized as follows: ~Sec.~\ref{sec:background} gives the background material.
Sec.~\ref{sec:sanitization} presents \SAN, the new technique for determining semantic relations.   
Sec.~\ref{sec:approach} gives an overview of our approach, \approach, for eliciting and analyzing normative requirements. 
Sec.~\ref{sec:evaluation} presents the evaluation of the effectiveness of \SAN and \approach.
Sec.~\ref{sec:relatedwork} overviews related work.
Sec.~\ref{sec:conclusion} concludes the paper and discusses future research directions.





==> Archive/introduction-jun-28.tex <==
\section{Introduction}
\label{sec:introduction}
% Context: normative requirements
Software systems interacting with humans become prevalent in domains such as transportation~\cite{Pham-et-al-16,Nagatani-et-al-21}, health and social care~\cite{Salceda-05,Laursen-et-al-22}. 
% example
For example, in the domain of healthcare~\cite{Salceda-05,Laursen-et-al-22}, helper robots are being used to assist patients with dressing. 
The deployment of such systems raises significant concerns in the realms of social, legal, ethical, empathetic, and cultural aspects (referred to as SLEEC) that must be addressed during development~\cite{townsend-et-al-2022, Bremner2019DFW, Burton2020HMP}. 
% example
% For instance, to avoid that a dressing robot reveals a patient's personal information. 
For instance, a helper robot might accidentally reveal patients' personal information without patients' consent.
To tackle these concerns effectively, normative requirements (\nNFRs) are defined, which are non-functional system requirements (NFRs) based on social, ethical, legal, cultural, or other relevant factors, \red{which restrict the acceptable range of system behavior that excludes the concerns}. 
% example
For instance, \nNFRs{} for a helper robot may specify that the patient's well-being and privacy are prioritized by promptly completing the dressing task, especially when the patient is underdressed. 
\red{\nNFRs{} are then used to inform all subsequent software engineering (SE) activities, such as design and architecture, testing and validation, and compliance and regulation. 
It is therefore important to carefully elicit them, and to validate them at an early stage, to avoid propagation of mistakes.}

\red{Similarly to non-functional requirements, three main types of inconsistencies — conflict, restrictiveness, and sufficiency — can arise during the elaboration of normative requirements. 
Additionally, a potential source of inconsistency, namely redundancy, can also occur. 
In the following, we will describe each of these issues.}

% Conflicting rules
\boldparagraph{Conflicting \nNFRs}
Typically, \nNFRs{} can be specified by multiple stakeholders independently~\cite{Lamsweerde-Darimont-Letier-98}. 
These stakeholders have different concerns, priorities, and responsibilities. 
Consequently, a common problem in non-functional requirements elicitation is the occurrence of \emph{conflicting} requirements~\cite{Shah-et-al-21}. 
In the context of \nNFRs{}, where multiple factors must be considered simultaneously (e.g., social and legal factors), conflicting requirements can also arise from different norms and factors~\cite{townsend-et-al-2022}, even if the requirements are elicited by a single stakeholder, such as a SLEEC expert.
% example
For the helper robot, the \nNFR{} of ``protecting patients privacy'' might create a conflict with ``patient claustrophobia'' requirement if the patients insist on keeping the curtains open while being dressed. 
It is important to identify these conflicts in the requirement elicitation stage.

% Restrictive
\boldparagraph{Restrictive \nNFRs}
Resolving conflicting requirements is challenging, it can lead to a too \emph{restrictive} set of \nNFRs{} that may not align with the goals of stakeholders. 
% example
For example, resolving conflicts between ``protecting patients' privacy'' and ``patient claustrophobia'' by mandating robots not to dress claustrophobic patients can be considered overly restrictive.
Striking the right balance is crucial in such situations. 
The resolution process should aim to address conflicts effectively without overly restricting the system's capabilities and its ability to achieve the initial goals.
It is therefore essential to maintain the focus on the system's primary objectives and ensure that the resolution does not compromise its functionality or intended purpose.

%Sufficient 
\boldparagraph{Sufficient \nNFRs}
\red{Alternatively, instead of ending up with too restrictive requirements, we may encounter a situation where we end up with normative requirements which are insufficient and fail to address the SLEEC concerns.
For instance, we might focus on addressing cultural and ethical concerns but inadvertently overlook the importance of addressing legal concerns.
It is crucial to determine whether the elicited requirements are \emph{sufficient} in addressing all relevant concerns.}
\hlTodo{TODO: add an example}

% Redundant requirements
\boldparagraph{Redundant requirements}
Different norms and factors can also share requirements, such as social and legal requirements often intersect by nature. 
% example
For example, a social requirement may state that the robot should respect the privacy of the patient, while a legal requirement may specify that the robot must adhere to relevant data protection laws and regulations. 
In such cases, the elicited requirement might be \emph{redundant}, which is not critical. 
\red{However, reducing unnecessary redundant requirements would simplify the validation and requirement reviewing process, and decrease the risk of inconsistency if one requirement is modified but the redundant one is not.}~\cite{Matsumoto-et-al-17}.

% Existing work
\boldparagraph{Existing work and the limitations}
When \red{validating} \nNFRs, prior research recommends using the SLEEC DSL, a state-of-the-art (SoTA) normative DSL, for specifying these requirements as \dsl{} rules~\cite{Getir-Yaman-et-al-23}.
For instance, some of the helper robot \nNFRs{} are expressed as \dsl rules in fig.~\ref{fig:examplefig}. 
Getir-Yaman et al.~\cite{Getir-Yaman-et-al-23} have proposed a technique based on model checking~\cite{Gibson-Robinson-et-al-14} to detect conflicts and redundancies among these rules. 
\red{Specifically, they identify if two rules exhibit conflicting responses when they share the same trigger.}
% example
For instance, consider the following two requirements: (r1)``When the patient requests to be dressed and the curtains are open, the robot must not dress the patient'' and (r2)``When the patient requests to be dressed, the robot must dress the patient within 2 minutes''. 
These requirements have conflicting responses given the same trigger, which is the ``patient's request to be dressed''.
\red{Similarly, Getir-Yaman et al. identify if two rules are redundant by examining rules that share the same trigger and intersect their responses.} 
% limitation
\red{Further validation of different conflict definitions is necessary to ensure a consistent set of rules.} 
\red{Existing preliminary work~\cite{feng-et-al-23-b} aattempted to identify conflicts and redundancies that arise given a trigger for all situations between multiple rules.
For example, let us consider the following three requirements: (r3) ``When the patient has fallen, call support'', (r4) ``When the patient has fallen, provide companionship to the patient'', and (r5) ``When you call support, leave the patient to not obstruct the space''. In this case, the requirement (r5) ``leave the patient when you call support'' conflicts with (r4) ``providing companionship'' when (r3) ``when you call support because the patient has fallen''.}
\red{However, other conflicts among \nNFRs{} remain not explored yet, specifically the ones occurring in specific situations. 
For instance, let us consider (r4') ``When the patient has fallen, provide companionship to the patient unless the patient is not deaf''. Here, the situation ``when the patient is deaf'' and the patient has fallen, a conflict arises.}
\red{This paper addresses the need to extend the identification of such conflicts.}

\boldparagraph{Conflicting, restrictive, sufficient, and redundant \nNFRs}
\hlTodo{TODO: remove the examples and instead refer to previous example, and name vacuous and situantional conflicts earlier.}
\red{In this paper, our focus is to further investigate whether a single \nNFR{} \emph{conflicts}, or is \emph{redundant}, with a set of \nNFRs. Furthermore, we also focus on studying whether a set of \nNFRs{} is too \emph{restrictive} to achieve the purpose of the system, and whether the set of \nNFRs{} is \emph{sufficient} to address the relevant SLEEC concerns.} 
%
\red{To further investigate whether a single rule conflicts with a set of rules, first,} we aim to determine if triggering the rule in any situation would lead to a violation of some other rule, resulting in a conflict. 
We refer to this as ``\emph{vacuous conflict}''. 
% example
For example, let's consider the two previous requirements (r1) and (r2) as an example of vacuous conflict. Indeed, triggering the patient's request to be dressed will lead to a violation in all situations. 
Additionally, we are interested in exploring whether a rule may interact with other rules in a contradictory manner, but only under specific situations.
These interactions can also lead to conflicts between different rules, which we refer to as ``\emph{situational conflict}''.
For instance, let's consider the following two requirements: (r6) ``When the patient requests to eat, feed the patient within one hour unless the patient must follow a specific diet, in which case, contact the doctor first'' and (r7) ``When the doctor is sleepy, do not contact the doctor for non-urgent matters''. \red{The two requirements are conflicting under the situation: the patient is hungry and must follow a specific diet, and the doctor is sleepy.}
%
To ensure that resolving \emph{vacuous} and \emph{situational} conflicts does not result in overly restrictive requirements, we propose to check whether the set of requirements is empty. 
In other words, we examine whether the intended purpose of the system can still be achieved given our \nNFRs. \red{Similarly, we can also check if the requirements are sufficient to exclude concerning behavior by checking the emptiness of their intersections.  }
%\green{NF: Emptiness check can also be used to determine if the concerns are sufficently blocked by the requirements. } \green{LM: If we add this, it can not be in restrictiveness, but we should add completeness, basically emptiness is the technique that we use to solve our problems, but what we solve is two different things, first whether the requirements are to restrictivie, and second whether the requirements are sufficient (so complete) to address the given concerns.}
%
Finally, we are interested in validating whether the resulting conflict-free rules are redundant with each other, as well as within themselves. 
Normative rules can be complex and composed of several defeaters, so we want to ensure that any redundant defeaters and rules are intentional.

% Contributions statement
\boldparagraph{Contributions} 
The paper makes three-fold contributions.
Firstly, it defines the identification of vacuous, situational-conflicting, restrictive, and redundant rules as satisfiability checking problems. Secondly, it proposes a formal tool called \tool that aids in the identification and diagnosis of these concerns when dealing with \nNFRs{} expressed as rules in the SoTA SLEEC DSL. 
\tool accomplishes this by translating the SLEEC DSL rules into \fol (first-order logic with quantifiers over relation object) and it utilizes the SoTA FOL* checker as a backend solver~\cite{feng-et-al-23}. 
Furthermore, \tool provides a non-technical diagnosis by highlighting the identified concerns within the input rules.
Finally, \tool includes a web interface~\cite{icse-tool}.
The artifact is available in~\cite{ICSE-Artifact}.


% Evaluation
\boldparagraph{Evaluation} 
\hlTodo{Add: sentence for the evaluation results.}


% Significance
\boldparagraph{Significance}
Checking \nNFRs{} for conflicts, restrictiveness, sufficiency, and redundancies in software engineering is essential for maintaining consistency %(e.g., conflicting requirements may lead to unpredictable or inconsistent outcomes)
, compliance% (e.g., proper resolution and adherence to applicable rules and regulations)
, efficiency% (e.g., redundant requirements can introduce unnecessary complexity and increase development and maintenance efforts)
, and risk mitigation% (e.g., addressing these issues proactively, software engineers can mitigate potential risks and enhance the overall quality and reliability of the software) 
in the development and maintenance of software systems. 
The diagnosis computed by \tool can be used by software engineers to (semi-)automatically generate and suggest patches to resolve redundancy, conflicts, and address concerns. 
The resulting conflict-free \nNFRs{} can be utilized by software engineers for designing and analyzing the system before deployment. 

% structure of the paper
The rest of this paper is organized as follows:
Sec.~\ref{sec:background} gives an overview of the SoTA normative \dsl and the \fol satisfiability checker. 
\hlTodo{TODO: agree on the structure of the paper and add it here.}
%Sec.~\ref{sec:specification} presents our extended domain-specific language, \dsle, and describes how it is translated into first-order logic with quantifiers over relational objects.
%Sec.~\ref{sec:redundancies-conflicts} provides definitions of redundant and conflicting rules.
%Sec.~\ref{sec:algo} describes the sanitization algorithm.
Sec.~\ref{sec:evaluation} presents the evaluation of the proposed approach's effectiveness.
Sec.~\ref{sec:conclusion} discusses  future research directions.  

%---------------------------------------------------------------------------------------------------------------
%-- Archive
%---------------------------------------------------------------------------------------------------------------

%\begin{itemize}
%    \item Start with non-functional requirements (RE, TSE, Empirical engineering, Workshops)
%    \item Defines qualities for these requirements
%    \item Check if expressible as \dsl rules (obligations which constraints only the future with continuous, or disjoints time windows.)
%    \item If not fully applicable, define subsets.
%    \item Goal: ``check if this is garbage''
%\end{itemize}

%\hl{Define normative requirements}

%\hl{Expressing the requirements as rules }

%\hl{Introduce the need of rules sanitization during and/or after the requirement elicitation process.} ~\cite{Lamsweerde-Darimont-Letier-98}

%\hl{Existing sanitization tool}

%\hl{Problem we solve in this paper}



==> Archive/introduction.tex <==
\section{Introduction}
\label{sec:introduction}
% Context: normative requirements
Software systems interacting with humans are becoming prevalent in domains such as transportation~\cite{Pham-et-al-16,Nagatani-et-al-21}, and healthcare~\cite{Salceda-05,Laursen-et-al-22}, e.g., helper robots aimed to 
%% example
%For example, in healthcare~\cite{Salceda-05,Laursen-et-al-%22}, helper robots are being used to 
assist patients with dressing. 
The deployment of such systems raises significant concerns in the realms of social, legal, ethical, empathetic, and cultural aspects (referred to as SLEEC), e.g., \blue{a helper robot accidentally leaking a patient's private personal information when dressing them with the curtains open.} 
%that must be addressed during development~\cite{townsend-et-al-2022, Bremner2019DFW, Burton2020HMP}. 
% example
% For instance, to avoid that a dressing robot reveals a patient's personal information. 
%For instance, a helper robot might accidentally reveal patients' personal information without their consent.
To exclude such concerns effectively, 
researchers~\cite{townsend-et-al-2022, Bremner2019DFW, Burton2020HMP} proposed to use \emph{normative requirements}, i.e., non-functional requirements (NFRs) that restrict the acceptable range of system behavior.
%to exclude these concerns effectively.
%To tackle these concerns effectively, \emph{normative requirements} (\nNFRs) are defined, which are non-functional system requirements (NFRs) that restrict the acceptable range of system behavior to exclude the concerns. 
% example
For instance, \nNFRs{} for a helper robot may specify that the patient's well-being and privacy are prioritized by promptly completing the dressing task, especially when the patient is underdressed. 
\nNFRs{} are then used to inform all subsequent software engineering (SE) activities, such as design and validation. 

% SLEEC DSL
Prior research recommended using \dsl, a state-of-the-art (SoTA) domain-specific language~\cite{KOSAR201677}, for specifying \nNFRs{} as \dsl{} rules~\cite{Getir-Yaman-et-al-23,Getir-Yaman-et-al-23b}. \dsl{} is very close to natural language and has proven accessible to stakeholders without a technical background (e.g., lawyers, ethicists or regulators). A rule in \dsl{} can be accompanied by one or more \emph{defeaters}, introduced using the `\textbf{unless}' construct. Defeaters specify circumstances that preempt the original response and can optionally provide an alternative response. For instance, a simple normative rule $r1$ for a helper robot that supports dressing tasks for elderly individuals can be encoded as ``\textbf{when} DressingStarted \textbf{then} DressingCompleted \textbf{within} 3 minutes \textbf{unless} curtainsOpened \textbf{or} doorsOpened \textbf{then} Close \textbf{within} 2 minutes \textbf{unless} \textbf{not} personAssent''.

%It is therefore important to carefully elicit them, and to validate them at an early stage, to avoid the propagation of mistakes.

% NFRs challenges
\hlTodo{(Todo: Focus on complexity of N-NFRs, and tell that they need to be evaluated, we start with no-domain no-application specific validation, namely ...)}
Elicitation and early stage validation of non-functional requirements (NFRs) in general presents a complex, time-consuming process that is susceptible to errors~\cite{Meth-et-al-13,Didar-et-al-2005}. 
Typically, \blue{NFRs} can be specified by multiple stakeholders independently~\cite{Lamsweerde-Darimont-Letier-98}. 
These stakeholders have different concerns, priorities, and responsibilities.  Thus, \emph{well-formedness} issues such as \emph{conflicts}~\cite{Shah-et-al-21}, \emph{redundancies}, or \emph{insufficiencies}~\cite{Paech-et-al-04,Matsumoto-et-al-17,feng-et-al-23-b,Getir-Yaman-et-al-23} can arise during the elaboration of  NFRs, and support for addressing this has been proposed~\hlTodo{cite}.
% {\bf MC:  and now something about getting rid of conflicts}
Resolving conflicts is essential for ensuring the validity of NFRs whereby
identifying or removing  unnecessary redundant \blue{NFRs} simplifies the validation and reviewing process and decreases the risk of inconsistency if one \blue{NFR} is modified but the redundant one is not~\cite{Matsumoto-et-al-17}.
\blue{\red{It is also} important to ensure that the NFRs \red{is \textit{sufficiently} strong to address relevant concerns while} \red{is not overly} \emph{restrictive} to prevent system from achieving its initial objectives}.  {\bf MC: prev sentence does not parse} \green{\textbf{\underline{New}: is it better?}} 

% N-NFRs complexity 
\nNFRs{} present two additional layers of complexity.
 Firstly, the process includes challenges due to the involvement of stakeholders who often lack technical expertise.  While this problem is shared with NFRs in general, \nNFR{} stakeholders include experts with very different backgrounds:  lawyers, social workers, ethics experts, etc., and conflicting or redundant requirements can arise from different norms and factors~\cite{townsend-et-al-2022} even if elicited by a single stakeholder!
 Secondly, the task becomes even more complex when capturing intricate non-monotonic conditions expressed via \emph{if, then, unless} and time constraints (e.g., \textit{act within 1 week}), which are often abundant in \nNFRs~\cite{knoks2020,brunero2022,townsend-et-al-2022,feng-et-al-23-b}. 

% example
For example, consider a helper robot with the \nNFR{} of ``protecting patients' privacy'' ($r1$), which might \emph{conflict} with a ``patient claustrophobia'' \nNFR{} if the patient insists on keeping the curtains open while being dressed. Additionally, a social \nNFR{} may require respecting patient privacy, while a legal \nNFR{} may specify adherence to data protection laws, potentially creating a \emph{redundancy}. Resolving these issues may lead to \nNFRs{} that no longer align with stakeholder goals, either being overly \emph{restrictive} or \emph{insufficient} to address SLEEC concerns comprehensively.
%, such as overlooking important empathetic concerns, e.g.,  not providing empathetic communication to comfort the patient.}
% {\bf MC:  I do not follow.  I also feel that this paragraph can be much tigher} \green{\textbf{\underline{Simplified}}}

% Existing work
%\boldparagraph{Existing work on \nNFR{} \CRRI}
% intro SLEEC DSL
Existing work has analyzed certain \CRRI properties, such as redundancy and conflicts, but limited to interactions between only two \dsl rules~\cite{Getir-Yaman-et-al-23}, or ignoring specific contexts~\cite{feng-et-al-23-b}.
%as they do not consider larger rule sets or broader contexts, leading to missed errors – 
%as illustrated in the example below.
For instance, consider three \nNFRs{} expressed as \dsl rules: ($r2$) ``\textbf{when} PatientFallen \textbf{then} CallSupport'', ($r3$) ``\textbf{when} PatientFallen \textbf{then} provideCompanionship \textbf{unless} patientNotDeaf.'', and ($r4$) ``\textbf{when} CallSupport \textbf{then} not provideCompanionship''. In this case, the $r4$ (`do not provide companionship when you call support') conflicts with $r3$ (`providing companionship') in the situation where  `the deaf patient and has fallen' ($r2$). 
This conflict could not be detected using existing approach~\cite{feng-et-al-23-b}, but it represents a genuine threat to the validity of \nNFRs.
Existing approach~\cite{Getir-Yaman-et-al-23} also do not offer debugging assistance.
%In this context, by considering the full set of \nNFRs{} with broader context, we would identify be able to detect the conflict in the previous example. 

In this paper, we propose a comprehensive approach to analyze and debug \nNFRs{} \CRRI by checking a broad range of well-formedness constraints, including redundancy, conflicts (accounting for different contexts), restrictiveness, and insufficiency. 
To the best of our knowledge, our solution is the first to provide such an extensive analysis and debugging approach for \nNFRs.

%\boldparagraph{Conflicting, restrictive, insufficient, and redundant \nNFRs}
%{\bf MC:  intro needs to be rewritten from here on.}
%\boldparagraph{\nNFR{} \CRRI problem tackled in this paper}
%{\bf MC : this text screams "incremental work".  We are not further investigating.  We found an important problem that prior work did not solve and are now solving it.}
%In this paper, our focus is to further investigate whether a single \nNFR{} \emph{conflicts}, or is \emph{redundant}, with a set of \nNFRs. Furthermore, we also focus on studying whether a set of \nNFRs{} is too \emph{restrictive} to achieve the purpose of the system, and whether the set of \nNFRs{} is \emph{insufficient} to address the relevant SLEEC concerns.
%
%To further investigate whether a single rule conflicts with a set of rules, first, we aim to identify both \emph{vacuous} and \emph{situational} conflicts.  {\bf MC:  seems redundant with previous point.  In general, this paragraph and next are very long and do not help.  I propose to do this by example, followed by a short statement of contributions.}
%
%Then, we are interested in validating whether the resulting conflict-free rules are redundant with each other. %, as well as within themselves.\green{alcc: what does conflict within a rule means? } \green{\textbf{Answer}: It is not conflict, but redundancy within a rule, for instance if the defeaters are redundants (we observed this in our NIER evaluation).} 
%Normative rules can be complex, comprising several defeaters, so we want to ensure that any redundant defeaters and rules are intentional.
%
%To ensure that resolving \emph{vacuous}/\emph{situational} conflicts and \emph{redundancies} does not lead to excessively \emph{restrictive} requirements, we propose to check whether the set of requirements is too restrictive. %(i.e., the system main purposes are in the acceptable set of behaviours). 
%In other words, we examine whether the intended purpose of the system can still be achieved while adhering to our \nNFRs. 
%
%Finally, we check if the requirements are \emph{insufficient} in preventing concerning behavior.
%By checking whether there is any possibility for concerning behaviors to occur while still adhering to the \nNFRs. This helps us determine if our \nNFRs{} alone are sufficient to effectively prevent concerning behaviors.
%

% oveview schema
\input{Sections/Fig-latex/fig-approach}

% Contributions statement

\boldparagraph{Contributions}
This paper makes the following contributions: (a) a method for identifying  \CRRI issues in \nNFRs{} expressed in \dsl by converting them into satisfiability checking problems;
(b) a method for generating a non-technical diagnosis that pinpoints the causes of \CRRI issues by analyzing the causal proof of (un)satisfiability;
 (c) a validation of the effectiveness of the approach
 over 9 cases studies and 233 rules written by YYY non-technical and technical stakeholders.  
 %Technical and non-technical stakeholders collaborated in writing the normative requirements for each case study. 
% The stakeholders found \red{A}\% of the identified \CRRI issues to be relevant, and our diagnosis allowed them to resolve \red{B}\% of these issues. The artifacts are available at~\cite{ICSE-Artifact}.}
{\bf MC:  do not forget to mention, later, where the artifacts are available, and the tool.}
 
 Our approach, \approach, is implemented in a tool \tool -- see Fig.~\ref{fig:overview}.   \tool 
 %introduces \approach, a formal and tool-supported approach (depicted in Fig.~\ref{fig:overview})  to identify and diagnose  \CRRI issues in \nNFRs{} expressed in \dsl.\\
%\indent (B) By treating \CRRI issues as satisfiability checking problemsIt provides a tool for effective by treating them as satisfiability checking problems.}\\ 
\indent
%Specifically, \approach tackles \CRRI issue identification by formulating them as satisfiability checking problems.} \\
%\indent \blue{(B) \approach includes \tool, a tool that performs the following tasks:
%(B.1) Translating 
translates \nNFRs{} expressed as rules in the SoTA \dsl~\cite{Getir-Yaman-et-al-23,Getir-Yaman-et-al-23b} into first-order logic with quantifiers over relational objects (\fol)\cite{feng-et-al-23};
checks their satisfiability using the SoTA \fol{} checker~\cite{feng-et-al-23}; and generates a non-technical diagnosis. 
%
%(B.3) Generating a non-technical diagnosis that pinpoints the causes of \CRRI issues by analyzing the causal proof of (un)satisfiability.
%(B.4) Providing a web interface~\cite{icse-tool} for ease of use.} \\
%\indent \blue{(C) Collected nine real-world case studies, encompassing forest protection plans to deployed collaborative robots in the industry. In total, there are \red{$155$} \nNFRs{} evaluated to assess the effectiveness of \approach{} for identifying \CRRI issues and the usability of the diagnosis for resolving them. 


% Significance
\boldparagraph{Significance}
%Ensuring \CRRI of \nNFRs{} is essential for maintaining consistency, compliance,  efficiency, and risk mitigation  in the development and maintenance of software systems. The diagnosis computed by \approach can be used by software engineers to (semi-)automatically generate and suggest patches to resolve redundancy, conflicts, and address concerns. 
A comprehensive approach for analysis and debugging of \nNFRs{} is crucial in developing modern systems that increasingly interact with humans.  We believe that we are  the first to provide such an approach, supporting stakeholders with varying levels of technical expertise. Importantly, the diagnosis computed by \approach can be used by software engineers to (semi-)automatically generate and suggest patches for resolving issues, thereby further assisting the stakeholders with the \nNFR{} engineering  process.

% structure of the paper
The rest of this paper is organized as follows:
Sec.~\ref{sec:background} gives the background material for our work.
Sec.~\ref{sec:problem} defines the \nNFR{} \CRRI problem that we tackle in this paper.
Sec.~\ref{sec:sanitization} describes our approach, \approach, to identify \nNFRs{} \CRRI issues using \fol satisfiability checking.
Sec.~\ref{sec:diagnose} presents our approach that utilizes the causal proof of (un)satisfiability to highlight the reasons behind the \CRRI issues (e.g., conflict).
Sec.~\ref{sec:evaluation} presents the evaluation of the proposed approach's effectiveness.
Sec.~\ref{sec:relatedwork} compares \approach to existing NFR \CRRI checking approaches.
Sec.~\ref{sec:conclusion} discusses future research directions.
%---------------------------------------------------------------------------------------------------------------
%-- Archive
%---------------------------------------------------------------------------------------------------------------

%\begin{itemize}
%    \item Start with non-functional requirements (RE, TSE, Empirical engineering, Workshops)
%    \item Defines qualities for these requirements
%    \item Check if expressible as \dsl rules (obligations which constraints only the future with continuous, or disjoints time windows.)
%    \item If not fully applicable, define subsets.
%    \item Goal: ``check if this is garbage''
%\end{itemize}

%\hl{Define normative requirements}

%\hl{Expressing the requirements as rules }

%\hl{Introduce the need of rules sanitization during and/or after the requirement elicitation process.} ~\cite{Lamsweerde-Darimont-Letier-98}

%\hl{Existing sanitization tool}

%\hl{Problem we solve in this paper}

%Sec.~\ref{sec:specification} presents our extended domain-specific language, \dsle, and describes how it is translated into first-order logic with quantifiers over relational objects.
%Sec.~\ref{sec:redundancies-conflicts} provides definitions of redundant and conflicting rules.
%Sec.~\ref{sec:algo} describes the sanitization algorithm.

==> Archive/sanitization-archove.tex <==
\section{Sanitization with \fol Satisfiability} \label{sec:sanitization}

\red{\textbf{--------------------------------- COMING SOON ---------------------------------}}

\subsection{Encoding \dsl Rules in \fol}

\subsection{Inconsistencies Check via Satisfiability}


\red{\textbf{-------------------------------------------------------------------}}

\hlTodo{TODO: Introduce the} \approach, \hlTodo{in a header, 1) defining and encoding the identification of the} \nNFR{} \hlTodo{inconsistencies as satisfiability problem, 2) analyze UNSAT core to pinpoint the causes.}

% header
In this section, we present how to identify normative rules conflicts (vacuous and situational), redundancy, restrictiveness and sufficiency (see Sec.~\ref{sec:problem}) using \fol satisfiability checking.

\subsection{Restrictiveness/Insufficiency Check via Satisfiability}\label{sec:emptycheck}
%Given a set of rules and facts in $\dsl$, we can check if the behavior permitted by the rules contains all the facts (representing the desirable behaviors) via an emptiness check:

\red{Given a rule set $\ruleset$ and a set of facts representing some desirable (e.g., system purpose) or undesirable behaviors (e.g., SLEEC concerns), we can determine whether the behaviour permitted by the rules $\ruleset$ contains these facts via emptiness check:}

% It can determine whether the behaviour permitted by the rules contains all of the facts. It can also determine whether the set of rules is sufficient for excluding some undesirable behavior, also described as facts.

\begin{definition}[Rule Emptiness Check]\label{def:emptiness}
Let a rule set $\ruleset$ and a set of facts $\facts$ 
% {\bf MC:  does it matter what this represents?  aren't you just defining the emptyness check, without a particular intention?}
be given. 
 The emptiness check of   $\ruleset$ with respect to $\facts$ is
$\lang{\ruleset} \cap \lang{\facts} = \emptyset$.
\end{definition}

% It can determine whether the behaviour permitted by the rules contains all of the facts. It can also determine whether the set of rules is sufficient for excluding some undesirable behavior, also described as facts.

To check emptiness \red{(Def.~\ref{def:emptiness})} of $\ruleset$ with respect to $\facts$, we can check the satisfiability of the \fol constraint, $\translate{\ruleset} \wedge \translate{\facts}$, where $T$ is the  \fol translation function  defined in Tbl.~\ref{tab:translate}. \red{We first present the encoding function $T$ and then prove its correctness in Thm.~\ref{thm:transcorrectness}.}
% {\bf MC:  how does this connect with definition 11?}
% \red{\bf NF: we first presents the encoding function $T$, and then proves $T$ is correct in Thm.~\ref{thm:transcorrectness} where defintion 11 is used.}

\begin{figure*}
    \begin{tabular}{lll}
                \centering            $T(\rulesyntax{\event \wedge \prop}{\dobg})$ & \multicolumn{2}{l}{$\rightarrow$ $\forall \obj{\event}: \Class{\event}\exists \obj{\measures}:\Class{\measures}(\obj{\measure}.\textit{time} = \obj{\event}.\textit{time} \wedge (T^{*}(\prop, \obj{\measures}) \Rightarrow T^{*}(\dobg, \obj{\measures})))$}  \\
                
                $T(\factsyntax{\event \wedge \prop}{\dobg})$ & \multicolumn{2}{l}{ $\rightarrow$ $\exists \obj{\event}: \Class{\event}\exists \obj{\measures}:\Class{\measures}(\obj{\measure}.\textit{time} = \obj{\event}.\textit{time} \wedge (T^{*}(\prop, \obj{\measures}) \wedge T^{*}(\dobg, \obj{\measures})))$} \\
                
                $T^{*}(\cobg_1 \otherwise \cobg_2 \ldots \cobg_n, \; \obj{\measures})$& \multicolumn{2}{l}{$\rightarrow$ $T^{*}(\cobg_1, \obj{\measures}) \vee \exists \obj{\measures}_j:\Class{\measures}(\textbf{Violation}(\cobg_1, \obj{\measures}, \obj{\measures}_j) \wedge T^{*}(\cobg_2 \otherwise \ldots \cobg_n, \obj{\measures}_j))$} \\

                $T^{*}(\neg \dobg, \; \obj{\measures})$& \multicolumn{2}{l}{$\rightarrow$ $\neg T^{*}(\dobg)$} \\

                $T^{*}(\prop \Rightarrow \obg,  \obj{\measures})$&  \multicolumn{2}{l}{$\rightarrow$ $\neg T^{*}(\prop, \obj{\measures}) \wedge T^{*}(\obg, \obj{\measures})$} \\

                $\textbf{Violation}(\prop \Rightarrow \obg,  \obj{\measures}, \obj{\measures}_j)$&  \multicolumn{2}{l}{$\rightarrow$ $T^{*}(\prop, \obj{\measures}) \wedge \textbf{Violation}(\obg, \obj{\measures}, \obj{\measures}_j)$} \\
                
                $T^{*}(\within{\event}{\term},  \obj{\measures})$&  \multicolumn{2}{l}{$\rightarrow$ $\exists \obj{\event}:\Class{\event}(\obj{\measures}.\textit{time} \le \obj{\event}.\textit{time} \le \obj{\measures}.\textit{time} + T^{*}(\term, \obj{\measures}))$} \\

                $\textbf{violation}(\within{\event}{\term},  \obj{\measures}, \obj{\measures}_j)$&  \multicolumn{2}{l}{$\rightarrow$ $ \obj{\measures}_j.\textit{time} = \obj{\measures}.\textit{time} + T^{*}(\term, \obj{\measures})  \wedge \neg T^{*}(\within{\neg \event}{\term},  \obj{\measures})$ } \\

                $T^{*}(\within{\neg \event}{\term},  \obj{\measures})$& \multicolumn{2}{l}{ $\rightarrow$ $\neg T^{*}(\within{\neg \event}{\term},  \obj{\measures})$} \\

                $\textbf{Violation}(\within{\neg \event}{\term},  \obj{\measures}, \obj{\measures}_j)$&  \multicolumn{2}{l}{$\rightarrow$ \makecell{$ 
                (\obj{\measures}.\textit{time} \le \obj{\measures}_j.\textit{time} \le \obj{\measures}.\textit{time} + T^{*}(\term, \obj{\measures})) \wedge \exists \obj{\event}:\Class{\event}(\obj{\measures}_j.\textit{time} = \obj{\event}.\textit{time})$  \\ $\neg (\exists \obj{\event}_1:\Class{\event} (\obj{\measures}.\textit{time} \le \obj{\event}_1.\textit{time} < \obj{\measures}_j.\textit{time}) )$}} \\
                
                $T^{*}(c, \obj{\measures})$ $\rightarrow$ $c$  &  $T^{*}(\measure, \obj{\measures})$ $\rightarrow$ $\obj{\measures}.\measure$ &  \\
                $T^{*}(-\term, \obj{\measures})$ $\rightarrow$ $-T^{*}(\term, \obj{\measures})$& $T^{*}(\term_1 + \term_2, \obj{\measures})$ $\rightarrow$ $T^{*}(\term_1, \obj{\measures}) + T^{*}(\term_2, \obj{\measures})$ & $T^{*}(c \times \term, \obj{\measures})$ $\rightarrow$ $T^{*}(c, \obj{\measures}) \times T^{*}(\term, \obj{\measures})$\\
                
                $T^{*}(\top, \obj{\measures})$ $\rightarrow$  $\top$ & $T^{*}(\term_1 > \term_2, \obj{\measures})$ $\rightarrow$  $T^{*}( \term_1, \obj{\measures}) > T^{*}( \term_2, \obj{\measures})$ & $T^{*}(\term_1 = \term_2, \obj{\measures})$ $\rightarrow$  $T^{*}( \term_1, \obj{\measures}) = T^{*}( \term_2, \obj{\measures})$\\
                $T^{*}(\neg \prop, \obj{\measures})$ $\rightarrow$  $\neg T^{*}( \prop, \obj{\measures})$& $T^{*}( \prop_1 \wedge \prop_2, \obj{\measures})$ $\rightarrow$   $T^{*}( \prop_1, \obj{\measures}) \wedge T^{*}( \prop_2, \obj{\measures}) $ & $T^{*}( \prop_1 \vee \prop_2, \obj{\measures})$ $\rightarrow$   $T^{*}( \prop_1, \obj{\measures}) \vee T^{*}( \prop_2, \obj{\measures}) $
                \end{tabular}  
\caption{Translation rules from \dsl to \fol. Given a \dsl rule $\srule$, $T$ translates $\srule$ to an \fol formula using the translation function $T^{*}$. The function $T^{*}$ recursively visits the elements (i.e., term, proposition and obligations) 
% \hl{Discuss (we did not define components, should we say ``element'' instead, because component is a strong word)} 
of $\srule$ and translates them into \fol constraints under a relational object $\obj{\measures}$ representing the measures when $\srule$ is triggered. } 
\label{tab:translate}
\end{figure*}

\begin{figure*}
\begin{tabular}{| c | c | c |}
\hline
\makecell{ID} & \makecell{\dsl $\srule$} & \makecell{\fol $\translate{\srule}$}\\
\hline
$\srule_{c}$ &
 \makecell{$\textbf{when} \textit{OpenCurtainRqt} \; \wedge \; \neg \textit{underDressed}$  \\ $\textbf{then} \within{\textit{CurtainOpen}}{\textit{30 (sec)}}$} & 
 \makecell{$\forall \obj{cr}: \Class{\textit{OpenCurtainRqt}}\exists\obj{\measures}:\Class{\measures}$\\
    $(\obj{cr}.\textit{time} = \obj{\measures}.\textit{time} \wedge (\neg \obj{\measures}.\textit{underDressed} \Rightarrow$ \\ $\exists \obj{co}:\Class{\textit{CurtainOpen}} \obj{cr}.\textit{time} \le \obj{co}.\textit{time} \le \obj{cr}.\textit{time} + 30))$}\\
    \hline
    $\srule_{c'}$ &
 \makecell{$\textbf{when} \textit{OpenCurtainRqt} \; \wedge \; \neg \textit{underDressed}$  \\ $\textbf{then} \within{\textit{CurtainOpen}}{\textit{20 (sec)}}$} & 
 \makecell{$\forall \obj{cr}: \Class{\textit{OpenCurtainRqt}}\exists\obj{\measures}:\Class{\measures}$\\
    $(\obj{cr}.\textit{time} = \obj{\measures}.\textit{time} \wedge (\neg \obj{\measures}.\textit{underDressed} \Rightarrow$ \\ $\exists \obj{co}:\Class{\textit{CurtainOpen}} \obj{cr}.\textit{time} \le \obj{co}.\textit{time} \le \obj{cr}.\textit{time} + 20))$}\\
    \hline 
    $\fact_{c}$ & \makecell{$\textbf{exists} \textit{OpenCurtainRqt} \; \wedge \; \neg \textit{underDressed}$} &  
    \makecell{$\exists \obj{cr}: \Class{\textit{OpenCurtainRqt}}\exists\obj{\measures}:\Class{\measures}$\\
    $(\obj{cr}.\textit{time} = \obj{\measures}.\textit{time} \wedge \neg \obj{\measures}.\textit{underDressed})$}\\
    \hline
    $\violation{\srule_{c}}$ & \makecell{$\textbf{exists} \textit{OpenCurtainRqt} \; \wedge \; \neg \textit{underDressed}$ \\
    $\textbf{while} \within{\neg \textit{CurtainOpen}}{\textit{30 (sec)}}$} & \makecell{$\exists \obj{cr}: \Class{\textit{OpenCurtainRqt}}\exists\obj{\measures}:\Class{\measures}$\\
    $(\obj{cr}.\textit{time} = \obj{\measures}.\textit{time} \wedge (\neg \obj{\measures}.\textit{underDressed} \wedge$ \\ $\neg (\exists \obj{co}:\Class{\textit{CurtainOpen}} \obj{cr}.\textit{time} \le \obj{co}.\textit{time} \le \obj{cr}.\textit{time} + 30)))$} \\
    \hline
    $\srule_{c\times}$ & \makecell{$\textbf{when} \textit{OpenCurtainRqt} \; \wedge \; \neg \textit{underDressed}$ \\
    $\textbf{then} \within{\neg \textit{CurtainOpen}}{\textit{40}}$} & \makecell{$\forall \obj{cr}: \Class{\textit{OpenCurtainRqt}}\exists\obj{\measures}:\Class{\measures}$\\
    $(\obj{cr}.\textit{time} = \obj{\measures}.\textit{time} \wedge (\neg \obj{\measures}.\textit{underDressed} \Rightarrow$ \\ $\neg (\exists \obj{co}:\Class{\textit{CurtainOpen}} \obj{cr}.\textit{time} \le \obj{co}.\textit{time} \le \obj{cr}.\textit{time} + 40)))$} \\
    \hline
\end{tabular}





\caption{Examples of \hl{normalized} \dsl rules and their \fol translations. \hlTodo{TODO: Add an example with otherwise}}
\label{fig:examplefig}
\end{figure*}

To translate \dsl rules and facts into \fol constraints, the signature of \dsl is mapped to the signature of \fol as follows: (1) every event $\event \in \events$ is mapped to a class of  relational object $\Class{\event}$; and (2) every measure $\measure \in \measures$ is mapped to a named attribute in relational objects of class $\Class{\measures}$. \red{The function $T$ then translates every \dsl rule $\srule $ to a \fol formula $\translate{\srule}$ such that $\lang{\srule}$ is not empty if and only if $\translate{\srule}$ is satisfiable. $T$ follows the semantics of normalized $\dsl$ (Sec.~\ref{sec:background}). To translate the \textit{fulfillment} relation  with respect to a time point $i$ (i.e., $\models_i$), $T$ uses helper function $T^*$ to recursively visit element of the \dsl rule (i.e., obligations, propositions and terms) and encode the condition of fulfillment with respect to the time point $i$ (represented by the input relational object $\obj{\measures}$). $T$ also uses helper function \textbf{Violation} to translate the condition for obligations and conditional obligations to be violated at some time point $j$ (represented by the input relational object $\obj{\measures}_j$). }

More specifically, \red{$T$ translates a rule}
$\rulesyntax{\event \wedge \prop}{\dobg}$ to the following constraint: whenever the triggering event $\event$ occurs ($\forall \obj{\event}:\Class{event})$, the measures are available 
(i.e., $\exists \obj{\measures}:\Class{\measures}\cdot \obj{\event}.\textit{time} = \obj{\measures}.\textit{time}$), and if the measures 
 satisfy the triggering condition ($T^{*}(\prop, \obj{\measures})$), then the obligation chain is fulfilled ($T^{*}(\dobg, \obj{\measures})$). 
Similarly, every fact is translated to the constraint "there exists an occurrence of an event $\event$ ($\exists \obj{\event}:\Class{event})$, while the measures are available 
(i.e., $\exists \obj{\measures}:\Class{\measures}\cdot \obj{\event}.\textit{time} = \obj{\measures}.\textit{time}$) where the condition $\prop$ is satisfied ($T^{*}(\prop, \obj{\measures})$), and the obligation chain is  fulfilled ($T^{*}(\dobg, \obj{\measures})$)".
% \red{Notice that   
%  the function translation $T$ uses the helper function $T^*$, which recursively translates every element
% % \hl{\textbf{Discuss}: (same here, element?)}
% of the \dsl  rule (i.e., obligations, propositions and terms) under the \textit{current} measures represented by the relational object $\obj{\measures}$}. \hl{\textbf{MC:}  why now?}

To ensure that no two different measures for the same time point exist, we introduce the \fol \textit{measure consistency axiom}: $\textit{axiom}_{mc} \gets \forall \obj{\measures}_1, \obj{\measures}_2: \Class{\measures} (\obj{\measures}_1.\textit{time} = \obj{\measures}_2.\textit{time} \Rightarrow \obj{\measures}_1 \equiv \obj{\measures}_2)$, where $\equiv$ is the semantically equivalent relational constraint that asserts equivalence of every attribute between $\obj{\measures}_1$ and $\obj{\measures}_2$.

 \red{We now state and prove the correctness of the \fol encoding for emptiness checking:}


\begin{theorem}[Correctness of the \fol translation]\label{thm:transcorrectness}
Let a set of rules $\ruleset$ and facts $\facts$ in \dsl be given. There exists a trace $\fos = (\eventocc{1}, \measureassign{1}, \timestamp{1}),$ $ (\eventocc{2}, \measureassign{2}, \timestamp{2}),$ $\ldots  (\eventocc{n}, \measureassign{n}, \timestamp{n})$ such that $\fos \in \lang{\ruleset} \cap \lang{\facts}$ if and only if $\translate{\ruleset} \wedge \translate{\facts} \wedge \textit{axiom}_{mc}$ has a satisfying solution $(\domain, v)$.
\end{theorem}
% {\bf MC:  I am sorry, I do not follow.  How does this connect to the measure consistency axiom?  and why is it an axiom?}

\begin{sop}
    We prove the forward direction by constructing a satisfying solution $(\domain, v)$ to $\translate{\ruleset} \wedge \translate{\facts}$ from the trace $\fos \in \lang{\ruleset} \cap \lang{\facts}$. For every state $(\eventocc{i}, \measureassign{i}, \timestamp{i}) \in \fos$, we follow the construction rules: (1) for every event $\event \in \eventocc{i}$, add a relational object $\obj{e}$ of class $\Class{e}$ such that $v(\obj{e}.\textit{ext}) = \top$ and  $v(\obj{e}.\textit{time}) = \timestamp{i}$; and (2) add a relational object $\obj{\measures}$ such that $\obj{\measures}.\textit{time} = \timestamp{i}$ and $v(\obj{\measures}.m) = \measureassign{i}(\measure)$ for every measure $m \in \measures$. We then prove that the constructed $(\domain, v)$ is a solution to   $\translate{\ruleset} \wedge \translate{\facts} \wedge \textit{axiom}_{mc}$. 

    We prove the backward direction by constructing  $\fos$ from a satisfying solution $(\domain, v)$ to $\translate{\ruleset} \wedge \translate{\facts} \wedge \textit{axiom}_{mc}$. The construction maps every relational object $\obj{\event}$ and $\obj{\measures}$ to some state $(\eventocc{i}, \measureassign{i}, \timestamp{i}) \in \fos$, where (1) $\event \in \eventocc{i}$ if $v(\obj{\event}).\textit{ext} = \top \wedge v(\obj{\event}).\textit{time} = \timestamp{i}$; and (2) $\measureassign{\measure} = v(\obj{\measures}.\measure)$ for every $\measure \in \measures$ if $v(\obj{\measures}).\textit{ext} = \top \wedge v(\obj{\measures}).\textit{time} = \timestamp{i}$. We then prove $\fos \in \lang{\ruleset} \cap \lang{\facts}$ 
    and conclude the proof. 
    % {\bf MC:  do you mean that this shows that this proposition holds?}
\end{sop}



\begin{example}
    Consider the \dsl rule $\srule_{c}$ in Example~\ref{example:syntax}. The translated \fol constraint $\translate{\srule_{c}}$  is shown in Fig.~\ref{fig:examplefig}. The  $\dsl$ formalization of the fact "a user request to open the curtain while she is not under-dressed" and its translation into \fol are also shown in 
    %can be formalized  in $\dsl$ ($\fact_{c}$) and translated to \fol as shown in 
    Fig.~\ref{fig:examplefig}. The \fol formula $\translate{\srule_{c}} \wedge \translate{\fact_{c}}$ has a satisfying solution $(\domain, v)$ where (1) $\domain = \{\obj{\measures}_1, \obj{\measures}_2,$ $\obj{\textit{OpenCurtainRqt}}, \obj{\textit{OpenCurtain}}\}$; (2) $v(o.\textit{ext} = \top)$ for every $o \in \domain$; and (3) $v(\obj{\measures}_1.\textit{underDressed}) = \bot \wedge v(\obj{\measures}_1.\textit{time}) = 1$; 
    $v(\wedge v(\obj{\measures}_2.\textit{time}) = 2$. The solution is mapped to a trace $\fos = (\{\textit{OpenCurtainRqt}\}, \measureassign{1}, 1),$ $(\{\textit{OpenCurtain}\}, \measureassign{2}, 3)$ where $\measureassign{1}(\textit{underDressed}) = \bot$. \red{The trace $\fos$} is contained in $\lang{\srule_{c}} \cap \lang{\fact_{c}}$, and thus $\lang{\srule_{c}} \cap \lang{\fact_{c}}$ is not empty.  {\bf MC : so?}
\end{example}


\subsection{Detecting Redundancy via Satisfiability}
Recall from Def.~\ref{def:redudent}, a rule is redundant in a given rule set if and only if removing the rule from the rule set does not affect the behavior of the rule set.
By Def.~\ref{def:redudent}, 
%a rule $\srule \in \ruleset$
%is redundant if removing  the rule from $\ruleset$ does not change the %behavior of $\ruleset$. Therefore, 
$\srule$ is not redundant if and only if there exists a trace $\fos$ such that $\fos \models \ruleset \setminus \srule$ and $\fos \not\models \srule$. \red{ Fortunately, we are able to construct facts, refer as \textit{violations}, to describe the set of traces that violates a given rule. 
}

\begin{lemma}[Violations]\label{lemma:concern}
    Let a rule $\srule = \rulesyntax{\event \wedge \prop}{\dobg}$ be given. A trace $\fos \not\models \srule$ if and only if $\fos \models \violation{\srule}$ where  \red{$\violation{\srule}$ is the fact asserting the occurrence of $\event$ and a time where $\prop$ holds while violating $\dobg$} (\red{\quoted{$ \factsyntax{\event \wedge \prop}{\neg (\dobg})$}}).  
    {\bf MC:  I cannot parse this!}
\end{lemma}

\begin{example}
    A concern derived from a \dsl rule $\srule_{c}$ (Example~\ref{example:syntax},
    %from example~\ref{example:syntax}. The concern derived from $\srule_{c}$, 
    $\violation{\srule_c}$, is shown in Fig.~\ref{fig:examplefig}.
\end{example}

Lemma.~\ref{lemma:concern} enables detection of redundancy via satisfibility:

\begin{theorem}[Redundancy via Satisfiability]\label{Thm:redviasat}
    Let a set of \dsl rules ($\ruleset$) be given. A rule $\srule \in \ruleset$ is redundant if and only if $\translate{\ruleset \setminus \srule} \wedge \translate{\violation{\srule}} \wedge \textit{axiom}_{mc}$ is UNSAT. 
\end{theorem}

\begin{proof}
    By definition of redundancy (Def.~\ref{def:redudent}), $\srule$ is redundant if and only if there does not exist a $\fos$ such that $\fos \in \lang{\ruleset \setminus \srule}$ and $\fos \not\models \srule$. By Lemma~\ref{lemma:concern}, $\srule$ is redundant if and only if there does not exist a $\fos$ such that $\fos \in \lang{\ruleset \setminus \srule} \cap \lang{\violation{\srule}}$. By Thm.~\ref{thm:transcorrectness}, $\srule$ is redundant if and only if $\translate{\ruleset \setminus \srule} \wedge \translate{\violation{\srule}} \wedge \textit{axiom}_{mc}$ is UNSAT .
\end{proof}

\begin{example}\label{example:redudentSAT}
    Consider the rule set $\ruleset = \{\srule_{c}, \srule_{c'}\}$ in Example~\ref{exmaple:redudent}. The derived concern of $\srule_{c}$ and its \fol translation is shown in Fig.~\ref{fig:examplefig}. The \fol formula $\translate{\srule_{c'}} \wedge \translate{\violation{\srule_{c}}}$ is UNSAT, and thus $\srule_{c}$ is redundant in $\ruleset$.
\end{example}

Given a rule set $\ruleset$, we examine every rule in $\ruleset$ and check whether the rule is redundant by checking \fol satisfibility according to Thm.~\ref{Thm:redviasat}. In addition to reporting a binary "yes" or "no" answer, we also provide a diagnosis (if the rule is redundant), computed from a causal proof of UNSAT, to highlight the causes of the redundancy (see Sec.~\ref{sec:diagnose}).
%We will present the diagnose in Sec.~\ref{sec:diagnose}



\subsection{Detecting Vacuous Conflict via Satisfiability}\label{sec:conflictingchecking}
Recall from Def.~\ref{def:dconflict} that a rule $\srule \in \ruleset$ is vacuously conflicting in $\ruleset$ if the behavior defined by $\ruleset$ ($\lang{\ruleset}$)  trace where $\srule$ is triggered. In other words, triggering $\srule$ any situation will lead to a violation of some rules (and thus cause a conflict). Therefore, we can determine if a rule is vacuously conflicting by describing the set of traces where $\srule$ is triggered as facts in \dsl, and then checking whether it intersects with $\lang{\ruleset}$ via emptiness checking (Sec.~\ref{sec:emptycheck}). 

\begin{definition}[Triggering]\label{def:ruletrigger}
    Let a \dsl rule $\srule = \rulesyntax{\event \wedge \prop}{\dobg}$ be given. The \emph{triggering} of rule, denoted as $\triggerfunc{\srule}$, is the \dsl fact $\factsyntax{\event \wedge \prop}{\top}$.
\end{definition}

\begin{lemma}\label{lemma:vcdef}
    Let a set of rules $\ruleset$ be given. A rule $\srule \in \ruleset$ is vacuously conflicting if and only if $\lang{\ruleset} \cap \lang{\triggerfunc{\srule}}$ is empty.
\end{lemma}

Lemma~\ref{lemma:vcdef} is a direct consequence of Def.~\ref{def:dconflict} and Def.~\ref{def:ruletrigger}, and it enables vacuous conflict detection via satisfiability:

\begin{theorem}[Vacuous Conflict as Satisfiability]\label{thm:vcdef}
    Let a set of rules $\ruleset$ be given. A rule $\srule \in \ruleset$ is vacuously conflicting if and only if $\translate{\ruleset} \wedge \translate{\triggerfunc{\srule}} \wedge \textit{axiom}_{mc}$ is UNSAT.
\end{theorem}

\begin{proof}
    By Lemma~\ref{lemma:vcdef}, $\srule$ is vacuously conflicting if and only if $\lang{\ruleset} \cap \lang{\triggerfunc{\srule}}$ is empty. The emptiness checking problem can be encoded as the satisfiability problem by Thm.~\ref{thm:transcorrectness}.
\end{proof}

 \begin{example}
     Consider the rule set $\ruleset = \{\srule_{c} , \srule_{c\times}\}$ in Example~\ref{example:dconf}. The rules $\srule_{c}$ and $\srule_{c\times}$ and their \fol translations are shown in Fig.~\ref{fig:examplefig}. $\triggerfunc{\srule}$ is $\factsyntax{\textit{OpenCurtainRqt} \wedge \neg \textit{underDressed} }{\top}$. The \fol formula $\translate{\srule_{c}} \wedge \translate{\srule_{c\times}} \wedge \translate{\triggerfunc{\srule_{c}}} \wedge \textit{axiom}_{mc}$ is UNSAT, and thus $\srule_{c}$ is vacuously conflicting in $\ruleset$ due to $\srule_{c\times}$.
  \end{example}
    

Given a rule set, we examine each rule  to determine whether it is vacuously conflicting by checking \fol satisfiability using Thm.~\ref{thm:vcdef}. In addition to providing a binary "yes" or "no" answer, we also generate a diagnosis (in case the rule is redundant) obtained from a causal proof of UNSAT. This diagnosis helps highlight the causes of the conflict. The details of the diagnosis are in Sec.~\ref{sec:diagnose}.




==> Sections/proto.tex <==
\subsection{Control study methodology}
Our primary objective in designing this experiment is to assess whether \framework enables faster convergence and yields better quality requirements compared to a traditional approach without the framework. 
% Eval 1 - 
Sanitizations with and without - how many new WFIs

% Eval 2 - 
Overall framework effectiveness, compared without

A) Consider existing manual Eliciation
Compare with Automatic elicitation without time
\#iterations, time 

B) New two case-studies:
    Measure time
    and others metrics

- bound time

% Example small: smart watch - measuring movemnets/

% Friday -

Metrics:
\#nbWFIS
\#time
\#number of mutual rules (non redundant)

% Record:
Each iteration, rules before, sanitizaton, rules after and time



Controlled Study Protocol: Evaluating the Effectiveness of \framework

\boldparagraph{Objective}
To assess whether \framework enables faster convergence and yields better quality requirements compared to a traditional approach without the framework.

Study Design:
    Participants:
        Two groups of participants with similar backgrounds and experience in requirement engineering.
        Group A (Control Group): Will use traditional methods for requirement gathering and analysis.
        Group B (Experimental Group): Will use \framework.

    Materials and Tools:
        Standardized set of requirement engineering tools for both groups.
        Access to \framework for Group B.
        Documentation and guidelines for both methods.

    Procedure:
        Preparation Phase:
            Train both groups on their respective methodologies.
            Provide identical requirement gathering tasks to both groups, relevant to a predefined project scenario.
        Implementation Phase:
            Allow each group to perform requirement gathering and analysis within a fixed time frame (e.g., 4 weeks).
            Monitor the progress and methodologies used by each group.
        Evaluation Phase:
            Assess the completeness, quality, and clarity of the requirements gathered by each group.
            Measure the time taken by each group to reach the final set of requirements.
            Conduct surveys or interviews to gather qualitative feedback from participants.

    Metrics:
        Time to convergence: Time taken to finalize the requirement set.
        Quality of requirements: Assessed based on clarity, completeness, and relevance.
        Participant satisfaction and ease of use: Based on post-study surveys.

    Data Analysis:
        Compare the time taken and quality metrics between the two groups.
        Analyze survey responses for qualitative insights.
        Use statistical methods to determine the significance of the results.

    Ethical Considerations:
        Ensure participant consent and confidentiality.
        Provide an option to withdraw from the study at any time.

    Limitations:
        The study may be influenced by the participants' prior experience.
        Results may vary based on the complexity of the project scenario.

    Expected Outcome:
        A comparative analysis of the effectiveness of \framework in accelerating requirement gathering and enhancing quality.

Reporting:

The results will be documented in a comprehensive report detailing the methodologies, findings, statistical analysis, and conclusions of the study.
Conclusion:

This protocol aims to provide a structured and unbiased comparison of \framework against traditional requirement engineering methods, to validate its efficacy in real-world scenarios.


==> Sections/response.tex <==
\setcounter{page}{1}
\renewcommand{\thepage}{\roman{page}}

\section*{Responses to the Reviewers}
We are grateful to the reviewers for their thorough examination of our work and their relevant remarks. We carefully considered the required changes and updated the paper accordingly. We hope that upon acceptance, we will have the opportunity to address additional suggested changes that were not mandatory for this revision, after having more time. In the revised submission, the newly added text is indicated in \blue{blue}. All required changes are listed below (in \red{red}), together with our responses (in black).

\smallskip
\noindent
\textbf{Response to the special requests from the metareview}

\begin{enumerate}
    \item[\red{1.}] \red{Improving both the motivation and the discussion about the implications of our proposed technique.}
    
[Response:]
In the introduction, we now define the concept of normative requirements, explaining that they encompass both Functional Requirements (FR) and Non-Functional Requirements (NFR), thereby illustrating their orthogonal nature. Further, we now provide a clear description of SLEEC, a DSL for normative requirements that is accessible to non-technical stakeholders, explaining our rationale for its consideration. Following this, we articulate the specific problem we address. Finally, we explicitly state the significance of our contribution to the RE community, which we hope will clarify the motivation behind our work and its potential implications.

    \item[\red{2.}] \red{Add further methodological details as described in the Reviews, which impairs verifiability and replicability.}

[Response:] To explain how the prompting strategy was defined and validated, we have added a subsection titled ``Prompting Engineering'' in Section~\ref{sec:sanitization}. This subsection describes the process we undertook to produce the prompts for querying the LLM in our \SAN technique.
To explain how the evaluation was conducted, we have expanded our evaluation section with a subsection clarifying the evaluation methodology (Section V-A). Additionally, we have highlighted where the artifacts necessary to reproduce our results can be found.


    \item[\red{3.}] \red{Take care of the presentation issues identified.}

[Response:] 
In Section~\ref{sec:background}, we have simplified the background description by removing formalization details and instead, providing examples to explain the concepts. In Section~\ref{sec:evaluation}, we have integrated the reviewers' feedback. Specifically, we have clarified the statement of RQ1, used 'cases' appropriately instead of 'case studies', and ensured that we do not over-generalize in the description of the evaluation outcomes.

\item[\red{4.}] \red{III-B(1): “For all relations, LLM-San asks the LLM to provide a justification before producing the final verdict. This simulates the forward-thinking process and prevents the LLM from retrofitting a justification for a random verdict.” – Any evidence to support this? If it’s just a theory/ assumption, that needs to be specified.}

[Response:] 
The evidence we have is based on the experiments we report in the paper; we now clarify  this point in Section~\ref{sssec:llminit}. We have observed during the development of prompts for LLMs that, if LLMs are tasked with the same or similar queries multiple times and prompted to provide justification before the final verdict, they are less likely to produce conflicting results and illogical justifications. %However, these observations are based on our specific experiments. To generalize these results  more systematic experiment specifically designed to explore this question would be necessary.



%\item \red{7. The paper does not discuss implications for both researchers and practitioners. In particular, I believe the paper must discuss applicability, in practice, of the proposed approach due to the computational and privacy issues that might be triggered by the use of large generative language models.}

%[Response:]
%Give the time for the computational issue, events and measures reflect capabilities of the robots that is visible to the user, there are not something that is private and not accessible. Also, any LLM can be used, a private company could use an LLM that would preserve privacy.

\item[\red{5.}] \red{Is SLEEC the first formal language for normative requirements?  I don’t think so, I think some of the Nomos work had a underlying formal language.}


[Response:]
SLEEC~\cite{Getir-Yaman-et-al-23}, while not the first formal language for normative requirements, it is the first DSL designed to be accessible to non-technical stakeholders. We have clarified this and added more details about SLEEC in the introduction. We would like to emphasize that the contribution of our paper extends beyond SLEEC itself. We introduce an LLM-based technique to identify semantic relations within normative requirements. And we propose an approach that  integrates this semantic-relation extraction technique with existing automated reasoning methods to perform a nuanced analysis of normative requirements well-formedness, uncovering potential issues (e.g., conflicts) through an understanding of underlying semantic relations that would  not be identified otherwise. We have now clarified this in the introduction.

\item[\red{6.}] \red{Concerns regarding non-technical stakeholders as co-authors of this paper}

[Response]
The authors are separated into those who participated in developing the approach and those who evaluated it. A clear separation was maintained throughout the project's lifecycle to ensure objectivity. Non-technical stakeholders, listed as co-authors, contributed significantly by constructing two new cases of normative requirements for real-world healthcare systems (i.e., Tabiat and Casper). They also devoted considerable time to evaluating the proposed approach. It is important to understand that the stakeholders who elicited the requirements are best positioned to assess the proposed semantic relations and to judge the relevance of identified well-formdness issues. We clarified this in  Section~\ref{sec:evaluation}.

\end{enumerate}



==> Sections/specification.tex <==
\section{Specification}
\label{sec:specification}

\boldparagraph{Syntax}
A \dsle signature is a tuple $(C, E, M, \iota, \gamma)$. $E$ is set predicate symbol for event, and  $C$ , $M$ are function symbols for constants and measures, respectively.  
The function $\iota: (C \cup E \cup M ) \rightarrow \mathbb{N}$ associate every function (and predicate) with an arity.  
Function $\gamma: (C \cup M) \rightarrow \{\mathbb{Z}, \mathbb{B}\}$ associate each function's output with a datatype. 
For simplifying the presentation, we assume \dsle supports only integer ($\mathbb{N}$) and boolean ($\mathbb{B}$) while scalars can be interpreted as integers under constraints. 
Using $\gamma$, we partition $M$ into $M^b$ and $M^i$ for the set of measure symbols with type $\mathbb{B}$ and $\mathbb{Z}$ respectively. Similarly, we partition $C$ into $C^b$ and $C^i$ based on constants' data type. 

Let \dsle signature $(C, E, M, \iota, \gamma)$ be given. Boolean ($t^b)$ and integer ($t^i)$, inductively as:
% following grammar rule (5-10) shown in Table~\ref{tab:sleec-gram}. \red{TODO: continue}
A \dsl rule (3) has the syntax \sleeckeyword{when} \textit{trigger} \sleeckeyword{then}  \textit{response}. The \textit{trigger} (4) of a rule is always an event symbol $e \in E$ with a Boolean term representing the condition. A \textit{response} (15) of a rule is the presence / absence of an event (\textit{occ}) followed by \textit{alternative} and \textit{defeaters}. 
The syntax of \textit{occ} (17), \textit{alternatives}(18) and \textit{defeaters} (19) is shown in~\ref{tab:sleecplus-gram}. 
Defeaters is a sequence of defeater, where each defeater has a Boolean term as its condition and a \textit{response} as its consequence. Defeaters can be nested since a defeater's response can have its own defeater. However, the maximum level of nesting must be finite (i.e., without recursive defeaters). A ruleset $R$ is a set of \dsle rules. 


\begin{table}[t]
    \centering
    \scalebox{0.65}{
        \begin{tabular}{l c l}
        \toprule
            specification &    & defBlock ruleBlock\\\toprule
            defBlock &   & \sleeckeyword{def\_start} definitions \sleeckeyword{def\_end}\\
            definitions &    & definition $|$ definition definitions\\
            definition &    & event $|$ measure $|$ constant\\
            event &   & \sleeckeyword{event} eventID \hln{[{\sleeckeyword{(}}parameters{\sleeckeyword{)}}]}\\
            \hln{parameters} &  & \hln{parameter $|$ parameter parameters}\\
            \hln{parameter} &  & \hln{boolParameter $|$ numParameter $|$ scalarParameter}\\
            \hln{boolParameter} &  & \hln{boolParamID: {\sleeckeyword{boolean}}}\\
            \hln{numParameter} &  & \hln{numParamID:} \underline{{\sleeckeyword{numeric}}}\\
            \hln{scalarParameter} &  & \hln{scalarParamID: scale} \\
            measure &   & boolMeasure $|$ numMeasure $|$ scalarMeasure \\
            boolMeasure &   & \sleeckeyword{measure} boolMeasureID \hln{[{\sleeckeyword{(}} parameters {\sleeckeyword{)}}]}: \sleeckeyword{boolean}\\
            numMeasure &   & \sleeckeyword{measure} measureID \hln{[{\sleeckeyword{(}}parameters{\sleeckeyword{)}}]}: \sleeckeyword{numeric}\\
            scalarMeasure &   & \sleeckeyword{measure} measureID \hln{[{\sleeckeyword{(}}parameters{\sleeckeyword{)}}]}: scale\\
            constant &   & \sleeckeyword{constant} constID [=value]\\
            %type &  ::= & \sleeckeyword{boolean} $|$ \sleeckeyword{numeric} $|$ scale\\
            scale &   & \sleeckeyword{scale} \sleeckeyword{(}scaleArgs\sleeckeyword{)}\\
            scaleArgs &    &  argID $|$ argID, scaleArgs\\\toprule
            ruleBlock &    & \sleeckeyword{rule\_start} rules \sleeckeyword{rule\_end}\\
            rules &    & rule $|$ rule rules\\
            rule &    & ruleID \sleeckeyword{when} trigger \sleeckeyword{then} response\\
            trigger &    & eventID \hln{[{\sleeckeyword{(}} bindings{\sleeckeyword{)}}]} $|$ eventID \hln{[{\sleeckeyword{(}} bindings{\sleeckeyword{)}}]} \sleeckeyword{and} boolExpr\\
            \hln{bindings} &  & \hln{binding $|$ binding bindings} \\
            \hln{binding} &  & \hln{boolParamID {\sleeckeyword{=}} boolParamValue} $|$ \hln{numParamID {\sleeckeyword{=}} numParamValue} $|$ \\
            &&\hln{scalarParamID {\sleeckeyword{=}} scalarParamValue}\\
            \hln{boolParamValue} &  & \hln{boolParamValueID $|$ boolExpr}\\
            \hln{numParamValue} & & \hln{numParamValueID $|$ numExpr} \\
            \hln{scalarParamValue} & & \hln{scalarParamValueID $|$ scalarTerminal}\\
            boolExpr & & boolTerminal $|$ negation $|$ binaryExpr \hln{$|$ quantificationE}\\
            \hln{quantificationE} & & \hln{{\sleeckeyword{(some}} eventID {\sleeckeyword{(}}bindings{\sleeckeyword{)}} {\sleeckeyword{where}} boolExpr{\sleeckeyword{)}}} %\hl{TODO:semantic}
            \\
            boolTerminal &  & \sleeckeyword{true} $|$  \sleeckeyword{false} $|$ boolMeasureID \hln{$|$ boolParamValueID} %\hl{TODO: add semantic constraint} 
            \\
            negation &  & \sleeckeyword{(not} boolExpr\sleeckeyword{)}\\
            binaryExpr &  & boolBinaryExpr $|$ numericBinaryExpr $|$ scaleBinaryExpr\\
            boolBinaryExpr & & boolExpr boolOp boolExpr\\   
            numericBinaryExpr & & numExpr relOp numExpr \\
            scaleBinaryExpr & & scaleTerminal relOp scalaTerminal \\
            numExpr & & numericTerminal $|$ numBinFunc \\
            numericTerminal & & value $|$ numMeasureID \hln{$|$ numParamValueID}\\
            numBinFunc & & numExpr numOp numExpr \\
            scaleTerminal & & argID $|$ scaleMeasureID \hln{$|$ scalarParamValueID}\\
            response &   & occ [alternative] [defeaters] $|$ \sleeckeyword{\{}occ [alternative] [defeaters]\sleeckeyword{\}} \\
            occ &    & [\sleeckeyword{not}] eventID [\sleeckeyword{within} value timeUnit] \\
            alternative &     &  \sleeckeyword{otherwise} response \\
            defeaters &    & defeater $|$ defeater defeaters\\
            defeater &   & \sleeckeyword{unless} boolExpr [\sleeckeyword{then} response] \\
            numOp &   & + $|$ - $|$ * \\
            relOp &    & $<$ $|$ $>$ $|$ $<>$ $|$ $<=$ $|$ $>=$ $|$ = \\
            boolOp &    & \sleeckeyword{and} $|$ \sleeckeyword{or} \\
        \bottomrule
        \end{tabular}
     }
    \caption{\dsle grammar. The extension from \dsl~\cite{Getir-Yaman-et-al-23} grammar is highlighted in green. \hl{(correct the highlight for the underlined numeric type)}}
    \label{tab:sleecplus-gram}
\end{table}
